Observability of Nonlinear Dynamical Systems over Finite Fields

This paper discusses the observability of nonlinear Dynamical Systems over Finite Fields (DSFF) through the Koopman operator framework. In this work, given a nonlinear DSFF, we construct a linear system of the smallest dimension, called the Linear Output Realization (LOR), which can generate all the output sequences of the original nonlinear system through proper choices of initial conditions (of the associated LOR). We provide necessary and sufficient conditions for the observability of a nonlinear system and establish that the maximum number of outputs sufficient for computing the initial condition is precisely equal to the dimension of the LOR. Further, when the system is not known to be observable, we provide necessary and sufficient conditions for the unique reconstruction of initial conditions for specific output sequences.

==> cdc_intro.tex <==
\section{Introduction}
Dynamical Systems over Finite Fields (DSFF) are a special class of dynamics where the state space of the system is a considered to be a vector space over a finite field $\ff$. Such systems arise in models of Boolean Networks, Communication and cryptographic protocols, Genetic and Biological Networks, Finite State Automata to name a few. This class of systems have been recently studied in detail from a dynamical systems point of view since the works of \cite{DCheng_STP2010}. When the dynamics is nonlinear, the problems of computing the solutions, deciding controllability, observability and optimal control are inherently hard problems as they require to solve nonlinear algebraic equations over finite fields \cite{RamSule}. In this work, we address the problem of observability of nonlinear DSFF. Observability for dynamics over Boolean Dynamics has been addressed in the works of \cite{Laschov2013,DCheng_2009Obs, ValcherObs2013, Weiss2018} and mainly depend on the semi-tensor product based approaches towards Boolean Dynamics developed in \cite{DCheng_STP2010}. These works though solve for the observability of nonlinear systems through a linear algebraic framework, requires computations over exponential size matrices which may lead to poor scalability with the dimension of the system. The work \cite{RamSule} provides an alternative linear theory for nonlinear DSFF through the Koopman operator framework without necessarily requiring exponential sized linear systems. In this work, we have a fresh look at observability of such nonlinear systems by defining a minimal linear realization (defined as the Linear Output Realization) of a nonlinear autonomous system using the Koopman operator. With this LOR, we aim to give necessary and sufficient conditions for observability of the dynamical system as well as guarantee upper bounds on the number of outputs required for unique reconstruction of the initial condition from the outputs. 
% Discrete time dynamics over a set containing a finite number of elements are fundamental in the field of Finite State Automata (FSA), Boolean networks to name a few and find applications in various engineering sciences such as genetic and biochemical networks, communication and cryptographic systems. Given a set $X$ of finite cardinality, a finite dynamical system (FDS) is defined through a map $F:X\to X$ in the following way 
% \begin{align}
%     \label{eq:FDS}
%     x(k+1) = F(x(k))
% \end{align}
% where $k \in \mathbb{Z}_+$ and $x(k) \in X \forall \ k$. The dynamical evolution of $x_0 \in X$ under the FDS (\ref{eq:FDS}) is the sequence 
% \[
% x_0, F(x_0),F^{(2)}(x_0),\dots, F^{(i)}(x_0),\dots
% \]
% where $F^{(i)}$ is the $i^{th}$ composition of $F$ with itself. In general any such FDS can be brought to a 
% and a dynamics 
\section{Preliminaries}
A nonlinear DSFF is represented as
\begin{align}
    \label{eq:DSFF}
    \begin{aligned}
    x(k+1) = F(x(k)) \\
    z(k) = g(x(k))
    \end{aligned}
\end{align}
where $x(k) \in \fn$, $z(k) \in \fm$, $F(x): \fn \to \fn$ and $g(x): \fn \to \fm$ are the state, output, state transition map and output map respectively. 
% When the maps $F$ and $g$ are linear, the DSFF is referred to as a linear-DSFF (LDSFF) and has the following state space representation 
% \begin{align}
%     \label{eq:LDSFF}
%     \begin{aligned}
%     x(k+1) = A x(k) \\
%     z(k) = C x(k)
%     \end{aligned}
% \end{align}
% where $A \in \fnn$ and $C \in \fmn$. 

\begin{definition}[Observable states]
A state $x_0 \in \ff^n$ is said to be observable, if there exists a positive integer $K$ such that $x_0$ is the unique initial condition of the output sequence $z(k)$ it generates, for $k = 0,\dots,K-1$. The smallest such $K$, denoted as $K_{x_0}$ is defined as the observability index of the initial condition $x_0$.  
%An output sequence $z(k),\dots,$, $k = 0,1,\dots,K$ is said to be an observable sequence if there exist an unique initial condition $x_0$ which generates this sequence. The interval $[0,K]$, where $K$ the smallest integer for which this output sequence becomes unique is defined as be the observability window of the output sequence.
\end{definition}
\begin{definition}[Observability, Observability index and Observability window of a system]
A system is said to be observable, if every initial condition $x_0 \in \ff^n$ is observable. For an observable system, according to Definition 1, there exists a unique $K_{x_0}$ for every initial condition $x_0$. The maximum $K = max\ K_{x_0}$ over all $x_0 \in \ff^{n}$, is called the observability index of the system and the interval $[0,K-1]$ is defined as the observability window of the system (\ref{eq:DSFF}).
%A system is said to be observable, if for every output sequence $z(k)$, there exists a $K_{x_0} < \infty$ such that the output sequence $z(k)$, $k = 1,\dots,K_{x_0}$ is observable according to Definition 1. For an observable system, the smallest interval $[0,K]$, where $K = \max K_{x_0}$ over all $x_0 \in \ff^n$ is defined as the observability window of the dynamics. 
\end{definition}
\begin{proposition}
For an observable time-invariant DSFF (\ref{eq:DSFF}), $K$ is always finite.
\end{proposition}
\begin{proof}\textcolor{blue}{
For a DSFF as in equation (\ref{eq:DSFF}) over $\ff_q^n$, the total number of points in the state space is finite and equal to $q^n$, and the outputs $y \in \ff_q^m$, and the output space contains $q^m$ distinct points. For a shift-invariant DSFF, any initial condition $x_0$ will either be visited periodically with period $\leq q^n$ or will settle down into a periodic orbit (with period $\geq 1$) under the dynamics of (\ref{eq:DSFF}) and hence ultimately periodic \cite{RamSule}. The corresponding output sequence is ultimately periodic too. In general, any output sequence contains two parts, the pre-periodic component and the periodic component. As the output space is finite, both the pre-periodic component and the period of the periodic component are finite. Given that the dynamics is shift-invariant, the initial conditions from the output has to be essentially computed from the outputs $z(k)$, $k = 0,1,\dots,K$, where $K$ is time instant corresponding to the first period of the output orbit after the pre-periodic component. Hence the number of outputs required for computing the initial condition is finite. \hfill \qed
}
%Given that the dynamics is shift-invariant, all the information about the initial condition is contained in the pre-periodic part or within the first period of the output sequence. 
\end{proof}
 
% \begin{definition}
% The dynamical system given in (\ref{eq:DSFF}) is said to be \emph{observable} if for every initial condition $x(0)$, there exists a $K$ such that every output sequence is an observable sequence.
% % if there exists a $k>0$, such that given any output sequence 
% % \begin{align}
% % \label{eq:OutputSeq}
% %     z(0),z(1), \dots, z(k-1)
% % \end{align} of length $k$, there exists a unique initial condition $x(0) \in \fn$ which generates the sequence (\ref{eq:OutputSeq}). 
% \end{definition}

When the system (\ref{eq:DSFF}) is linear with state transition matrix $A$ and output matrix $C$, a necessary and sufficient condition for the system to be observable is that the following matrix $\mco$ (known as the \emph{Observability matrix}) 
\begin{align}
\label{eq:Obsmat}
    \mco = \begin{bmatrix}C \\ CA \\ \vdots \\ CA^{n-1}\end{bmatrix}
\end{align}
is full rank and the corresponding initial condition $x_0$ which generates the given sequence is the solution of the following system of linear equations
\begin{align}
\label{eq:ObsEqLin}
\mco x_0 =  \begin{bmatrix} z(0) \\ z(1) \\ \vdots \\ z(n-1) \end{bmatrix}.
\end{align}
In linear systems, as a consequence of Cayley Hamilton Theorem, at most $n$ output instances are required to compute the corresponding initial condition $x_0$. In general, for a multi-output linear system, if the system is observable, the observability window can be computed as $[0,n_o - 1]$, where $n_o$ is the observability index\footnote{The observability index of a linear system is the minimal $k$ such that $CA^{k}$ is linearly dependent on the previous iterates $CA^{i}$.} of the system. Also, it can be seen that for linear systems, observability of one state guarantees the observability of the entire state space (and hence the system itself). 
 \begin{proposition}
 In a linear system, observability of one particular initial condition is equivalent to observability of the entire system. 
\end{proposition}
 \begin{proof}
 \textcolor{blue}{Given that a specific initial condition $x_0$ is observable from its output sequence $z(0),z(1),z(2),\dots,z(n-1)$. Then $x_0$ is the unique solution to the system of equation (\ref{eq:ObsEqLin}. Suppose the system is unobservable, then $\mco$ is singular and there exists a nontrivial kernel $\mathcal{N}(\mco)$. Let $w \in \mathcal{N}(\mco)$, then we know that 
 \[
 \mco (x_0 + w) = \mco x_0
 \]
 and $x_0+w$ is also a solution of (\ref{eq:ObsEqLin}) which contradicts the observability of $x_0$. 
}
\end{proof}

We denote by $\mz$, the output sequence $z(k)$ of arbitrary length, and by $\mz_K$ an output sequence of length $K$ at time instants $0,1,\dots,K-1$.
\begin{definition}[Observability of an output sequence]
An output sequence $\mz_K$ of length $K$ is said to be observable if there exists an unique initial condition $x_0$ which generates the sequence.     
\end{definition}
This notion of observability is defined from the context of a specific output sequence of length $K$ rather than from the context of the initial condition. It can be seen that both these definitions are interchangeable: When a initial condition is observable, its corresponding output sequence $\mz_{K_{x_0}}$ is also observable, where $K_{x_0}$ is the observability index of $x_0$. If the system is observable, it can be seen that every output sequence $\mz_K$ is observable where $K$ is the observability index of the system. The idea of looking at the observability of a system from the output sequence is important because in many practical applications, it is necessary to ascertain the uniqueness of the initial condition for a given output sequence $\mz_K$ of length $K$. 

% does not have an unique solution $\tx$. This means that the matrix $\mco$ is not full rank and there exists a non-zero vector $\alpha \in ker\ (\mco)$. This also means that 
% \[
% \mco (x_0 + \alpha) = \mco x_0 + \mco \alpha = \begin{bmatrix} z_0 \\ z_1 \\ \vdots \\ z_{n-1} \end{bmatrix}
% \]
% which contradicts the uniqueness of $x_0$ corresponding the sequence $z_0,z_1,\dots,z_{n-1}$. 

\subsection{Challenges in Observability of a nonlinear DSFF}
For a nonlinear DSFF, determining the observability of an initial condition $x_0$ involves establishing existence of a positive integer $K$ such that the following system of algebraic equations (\ref{eq:ObsEq}) has $x_0$ as the unique solution. 
\begin{align}
\label{eq:ObsEq}
\begin{aligned}
    z(0) &= g(x_0) \\
    z(1) &= g(F(x_0) \\
    & \ \ \vdots \\
    z(k-1) &= g(F^{(K-1)}(x_0))
\end{aligned}
\end{align}
where $F^{(j)}$ is the $j^{th}$ composition of $F$ with itself 
\[
F^{(k)} = \underbrace{F \circ F \circ \dots \circ F}_{j\ \text{times}}.
\]
Computing $x_0$ and establishing its uniqueness for a given output sequence as in (\ref{eq:ObsEq}) is called the \emph{observability problem}. Computing the solution of the nonlinear system of equations (\ref{eq:ObsEq}) over a finite field $\ff$ is an inherently hard computational problem. We highlight the challenges in determining observability of a nonlinear DSFF.
\begin{enumerate}
    \item Solving for multivariate polynomial equations (\ref{eq:ObsEq}) over finite fields is an $NP$-hard problem \cite{LB_Hybrid2009}. No known efficient algorithm exists for general finite fields. Computer algebraic approaches based on Gr\"{o}bner basis techniques can be used for computing such solutions, however these techniques are not known to be efficient to scale up with the dimension of the system.
    \item For a given output sequence $\mz_K$, it is guaranteed that there exists atleast one initial condtion $x_0$ as a solution of (\ref{eq:ObsEq}). It is however pertinent to ascertain the uniqueness of the solution $x_0$ to (\ref{eq:ObsEq}), because existence of a solution $x_0$ does not guarantee observability of that output sequence.
    \item The definition of observability of a dynamical system implicitly involves the length of the observability window $[0,K-1]$ which guarantees the uniqueness of $x_0$. This window is well defined for linear systems and equal to $[0,n_o-1]$, where $n_o$ is the observability index. For a general nonlinear dynamics, there are no specific results on the upper bound on $K$. A result on the estimate of $K$ is important for deciding observability of output and computation of the initial conditions. 
    
    %For a general nonlinear dynamics, there are no specific results on the existence or bounds on $K$. Such a result is important as the knowledge of $K$ can help in determining the sufficient number of outputs required for deciding on the unobservability of the system (or a specific initial condition or an output sequence). 
    \item Unlike in linear systems, where observability of a single initial condition (or a single output sequence) guarantees the observability of all initial conditions (or of all output sequences), nonlinear systems may have certain initial conditions (or output sequences) to be observable while other initial conditions (or output sequences) may not be observable. So uniqueness of the solution $x_0$ for a particular output sequence $\mz$ does not guarantee uniqueness of initial conditions of all output sequences and this makes characterizing the observability of the entire system difficult.
    % %\item The definition of observability %does not explicitly define the time instances 
    % also implicitly involves the length $k$ of output sequences upto which %the measurement is needed for
    % the outputs need to be known for guaranteeing %observability of the output sequence.
    % existence of an unique $x_0$. For linear systems of dimension $n$, it is known that any output after the $n^{th}$ time instant is not necessary for the computation of initial condition $x_0$. No such upper bounds are available at present for nonlinear systems which makes it difficult to characterize observability condition. 
    
\end{enumerate}

With the above motivations for the observability of nonlinear DSFF, in this paper we have a fresh look at the observability problem through the Koopman Operator framework. 

\subsection{Koopman Operator Framework for DSFF}
Consider the space of functions $\Vo$ of scalar valued functions $\psi : \fn \to \ff$. This space is of finite dimension (and equal to $q^n$) when $\ff$ is the finite field $\ff_q$. The \emph{Koopman operator} $\Koop$ \cite{Koopman} associated with the dynamics (\ref{eq:DSFF}) is defined as 
\begin{align}
\label{eq:KoopmanOp}
    \Koop \psi = \psi \circ F
\end{align}
This map $\Koop$ is linear over $\Vo$. Starting from a function $\psi \in \Vo$, one can define the sequence 
\[
\psi, \Koop \psi := \psi(F), (\Koop)^2 \psi := \psi(F^{(2)}),\dots
\]
The iterates of the above sequence can be visualized as the evolution of the following dynamical system 
\begin{align}
\label{eq:KLS}
\psi_{k+1} = \Koop \psi_{k}
\end{align}
starting from $\psi_0 = \psi$. The system (\ref{eq:KLS}) is over $\Vo$ and is $\ff$-linear and defined as the \emph{Koopman linear system} (KLS) for the dynamical system (\ref{eq:DSFF}). The work \cite{RamSule} establishes the relationships between the nonlinear DSFF and the KLS. 

This paper focuses on the solution to the observability problem (\ref{eq:ObsEq}) and develops a necessary and sufficient condition for observability of the nonlinear DSFF through the Koopman operator framework by restricting it to a specific invariant subspace of $\Vo$. 



==> obs_LOR.tex <==
\section{Observability of the DSFF through LOR}
% Given a DSFF as in (\ref{eq:DSFF}) and its corresponding LOR (\ref{eq:LOR}), to establish algebraic conditions for the observability of the original nonlinear system using the LOR, we define a specific set of functions in the space $\Vo$ called the coordinate functions as follows
% \begin{definition}
% The function $\chi_i(x) \in \Vo$ defined as 
% \[
% \chi_i(x) = x_i 
% \]
% is called the \emph{i-th coordinate function}
% \end{definition}
Given $\Vo$ over $\ff^n$, let $\chi_i(x) \in \Vo $ be the $i^{it}$ coordinate function defined as
\[
 \chi_i(x) = x_i.
\]
The state of the system at a point $x_0 \in \ff^n$ is the evaluation of the $n$-tuple of coordinate functions $\hchi = [\chi_1,\dots,\chi_n]^T$ at $x_0$. Unique reconstruction the initial state $x_0$ of the DSFF from the output sequence is equivalent to unique reconstruction of the $\hchi$ at $x_0$ from the output sequence. The following result characterize the observability of the nonlinear DSFF through the LOR.

\begin{theorem}
\label{thm:obs_phat}
The DSFF is observable iff the map $\phat: \ff^n \to \ff^N$ defined in (\ref{eq:phat}) is an injective map of $\ff^n$ into $\ff^N$. 
\end{theorem}
\begin{proof}
(Sufficiency): Given that the map $\phat$ is an injection, for every $\phat(x_0) \in \ff^N$, there exists an unique $x_0 \in \ff^n$. Consider any output sequence $z(k)$ of the DSFF. For the assignment $\tz(k) = z(k)$ of the LOR and using the fact that the LOR is observable, there exists an unique $y_0$ satisfying $y_0 = \phat(x_0)$. Under the assumption that $\phat$ is $1-1$, there exists an unique $x_0$ corresponding to the output sequence $z(k)$ of the DSFF which proves that the DSFF is observable. 

(Necessity): Given that the DSFF is observable, for every output sequence $z(k)$, there exists an unique $x_0$ which generates that sequence. When LOR is initiated with $\phat(x_0)$, the output sequence $\tz(k)$ of the LOR is identical to the output sequence $z(k)$ of the DSFF. Since LOR is observable, the initial condition $\phat(x_0)$ is unique for a given output sequence. Hence the map $\phat(x_0)$ is $1-1$ as each $x_0$ generates an unique output sequence $z(k)$.
\end{proof}

% \begin{lemma}
% Given a DSFF over $\ff$ as 
% \begin{align}
% \label{lem:1var}
% \begin{aligned}
%     x(k+1) &= f(x(k)) \\
%     z(k) &= g(x(k))
% \end{aligned}
% \end{align}
% where $x(k),z(k) \in \ff$. The DSFF is observable if $g(x)$ is a bijection over $\ff$. 
% \end{lemma}
% \begin{remark}
% The above lemma is necessary to isolate those dynamical systems where the internal dynamics has no role in the observability. When the output $g$ is a bijection of the state space, there exists a unique $x_0$ for every $g(x_0)$. This guarantees the observability of the dynamical system. 
% \end{remark}
% \textcolor{blue}{\begin{remark}
% Observability is an intrinsic property of the map from $\ff^n \to W$ for a given nonlinear DSFF and it is to be noted that choice of the basis functions $\mcb$ in equation (\ref{eq:phat}) does not affect the observability of the system. Also, given two (un)observable nonlinear DSFFs related by a nonlinear transformation of the state space, from Lemma \ref{lem:NS_Transform}, their (un)observability is preserved too in their corresponding $\phat$.
% \end{remark}}

\begin{corollary}
\label{cor:DSFF-obs_suf}
The DSFF is observable if all the coordinate functions are in $W$
\end{corollary}
\begin{proof}
Given all the coordinate functions are in $W$, there exists a unique matrix $C \in \ff^{n \times N}$ such that 
\begin{align}
\label{eq:statemap}
\hchi = C \phat 
\end{align}
% Since DSFF is observable, for every sequence $z(k), k=0,1,\dots$, there exists an unique $x_0$. 
From LOR and Proposition \ref{prop:OE}, we know that if LOR is initialized with $\phat(x_0)$, then $z(k) = \tz(k)$. To compute this $\phat(x_0)$, we solve for 
\[
\begin{bmatrix} \tz(0) \\ \tz(1) \\ \vdots \\ \tz(N-1) \end{bmatrix} = \mco \phat(x_0) 
\]
with $\tz(k) = z(k)$. Since LOR is observable, there exists a unique $\phat(x_0)$ for each output sequence $z(k)$. This unique $\phat(x_0)$ gives the unique $x_0$ through equation (\ref{eq:statemap}) as
\[
x_0 = \hchi(x_0) = C \phat(x_0)
\]
which is the unique initial condition corresponding to the output $z(k)$. 


% (Necessity): To prove the necessity, we use the result in Lemma \ref{lem:obs_phat}. From the lemma we assume the map $\phat(x)$ is $1-1$. We prove that $\phat(x)$ being $1-1$ implies that the coordinate functions are in the linear span of $\mcb$. 

% Since DSFF is observable, there exists an unique $x_0$ for each output sequence $z(k)$. Also from the observability of the LOR, there exists an unique $y_0 = \phat(x_0)$ for a given output sequence $z(k)$. This means that for each $\phat(x_0)$, there exists an unique $x_0$. As we know that $\phat = [\psi_1,\dots,\psi_N]^T$ and each of these $\psi_i$ are functions from $\ff^n \to \ff$, they can be written as a unique linear combination of monomials in $\{x_1,\dots,x_n\}$. The list of monomials contains elements of the type
% \[
% \mu(i) = x_{1}^{i_1} x_{2}^{i_2} \cdots x_{n}^{i_n}
% \]
% where $i = (i_1,\dots,i_n)$ and $0 \leq {i_j} \leq q-1$. Let $\hM(x)$ be the column vector of all monomials, where we fix the first $n$-rows as the degree 1 monomials and then add all other monomials (including the constant term) in the later rows with increasing degrees. The column vector $\hM(x)$ is of size $q^n$. There exists a unique matrix $A \in \ff^{N \times q^n}$ such that 
% \begin{equation}
% \phat (x) = A \hM(x)
% \label{eq:temp2}
% \end{equation}
% where the matrix $A$ is a wide matrix with rank atleast $n$. This is because the map $\phat$ is $1-1$ over $x \in \ff^n$ and hence the matrix $A$ must have atleast $n$ linearly independent columns. Also the rank of $A$ is at most $N$ (since $N \leq q^n$). So there exists a sequence of column operations leading to 
% \[
% A \to [A_1 \ \ 0]
% \]
% where $A_1 \in \ff^{N \times r}$ is a full rank matrix, where $r$ is the rank of $A$. Effectively, the system of equations (\ref{eq:temp2}) can be written as 
% \[
% \phat(x)  = [A_1 \ \ 0] \begin{bmatrix}M_r \\ \bar{M_r} \end{bmatrix}
% \]
% where $M_r$ is the first $r$ monomials in the list of monomials. This $M_r$ contains the monomials of degree $1$ by construction. This gives a reduced set of equations 
% \[
% \phat(x) = A_1 M_r(x)
% \]
% and since $A_1$ is full rank, there exists a left inverse $A_1^\dagger$ leading to 
% \[
% M_r(x) = A_1^\dagger \phat(x)
% \]
% This proves that the monomials in $M_r$ are in the linear span of $\phat$. Each of the coordinate functions $\chi_i(x)$ is the monomial $x_i$ and hence the coordinate functions are in the span of $\phat$. 


% The set $\{x_1,x_2,\dots,x_n\}$ (i.e., the monomials of degree 1) form a subset of the monomials. Let $M_m = [x_1,\dots,x_n]^T$ be the vector of such degree $1$ monomials. Then the matrix $A$ in equation (\ref{eq:temp2}) has a submatrix of $n$-columns $A_1$ which multiply this vector of degree 1 monomials. The equation can be written as 

% % the equation (\ref{eq:temp2}) can be rewritten as 
% % \[
% % \phat(x) = [A_1 \ \ A_2] \begin{bmatrix}
% % M_m \\ \hM-\{M_m\} \end{bmatrix}
% % \]
% % where $\hM-\{M_m\}$ is the elements of the set $\hM$ apart from the degree $1$ monomials. We know by observability of the DSFF, for every $x_0 \in \ff^n$, there exists an unique $\phat(x_0)$. This means that the two system of equations 
% % \[
% % \phat(x) = A_1 M_m \ \ \quad \ \ \phat(x) = A_2 (\hM-\{M_m\})
% % \]
% % \[
% % \phat(x) = A_1 M_m + \phat_1(x)
% % \]
% We see that $M_m = [x_1,\dots,x_n]^T = [\chi_1,\dots,\chi_n]^T(x) = \hchi(x)$. So, 
% \[
% \phat(x) = A_1 \hchi(x)
% \]
% and this has an unique solution for each $x \in \ff^n$. This means that $A_1$ is full row rank and hence there exists a left inverse $A_1^* \in \ff^{n \times N}$ such that $A_1^* A_1 = Id_{n}$. This gives  
% \[
% \hchi(x) = A_1^* \phat(x)
% \]
% and hence each $\chi_i$ is in the linear span of the basis functions. 
\end{proof}
  
% \begin{theorem}
% The DSFF is observable only if the the coordinate functions are in the ideal generated by the basis functions $\psi_j(x)$.
% \end{theorem}

% \
% \begin{remark}
% If the coordinate functions are in the span of the basis functions $\psi_j(x)$, then the entire polynomial ring $\ff[x_1,\dots,x_n]$ is generated by $\psi_j(x)$. 
% \end{remark}
The following result establishes the connection between the number of outputs required for unique reconstruction of the initial condition and the dimension of the LOR. Such a result is important for establishing computational bounds on the observability problem of nonlinear DSFF.
\begin{theorem}
\textcolor{blue}{Given an observable DSFF (\ref{eq:DSFF}) and its corresponding LOR (\ref{eq:LOR}) then the DSFF is observable in the interval $[0,N-1]$ and the observability window of the DSFF is $[0,N-1]$.}
\end{theorem}
\begin{proof}
\textcolor{blue}{As the DSFF is observable, then there exists a $K > 0$ such that following set of equations have a unique solution $x_0$
\begin{align}
\label{eq:ObsK}
\begin{aligned}
z(0) &= g(x_0) \\ 
z(1) &= g(F^{(1)}(x_0)) \\
&\ \ \vdots  \\
z(N-1) &= g(F^{(N-1)}(x_0)) \\
z(N) &= g(F^{(N)}(x_0)) \\
&\ \ \vdots \\
z(K-1) &=g(F^{(K-1)}(x_0)) \\
\end{aligned}
\end{align}
From the recurrence relation defined in (\ref{eq:Op-rec}), we can eliminate the last $K-N$ equations by taking linear combinations of the first $N$ equations and hence the above system of equation reduces to the form 
\begin{align}
\label{eq:ObsEqns}
\begin{aligned}
z(0) &= g(x_0) \\ 
z(1) &= g(F^{(1)}(x_0)) \\
&\ \ \vdots  \\
z(N-1) &= g(F^{(N-1)}(x_0))
\end{aligned}
\end{align}
From the observability of the DSFF, we know that the above equation has an unique initial condition $x_0$ for every output sequence of the system. This proves the first statement.}

\textcolor{blue}{The second statement can be proved as a consequence of Theorem \ref{thm:obs_phat} and Lemma \ref{lem:LOR-obs}. To uniquely determine $\phat(x_0)$, $y_0$ corresponding to the output sequence has to be computed as in (\ref{eq:phat1}). Since the LOR is observable, the minimum number of outputs required to uniquely compute the initial condition is $N-1$. Hence the DSFF is not observable for any interval $[0,N_1]$, where $N_1 < N-1$. }



% To prove the second statement, consider a basis of $\Vo$ over $\fqn$ to be $\{\phi_1,\dots,\phi_{q^n}\}$\footnote{One such basis can be all the monomials of the form $\prod_{i = 1}^n x_i^{d_i}$, with degrees $d_i \leq$ q.}. Every function $g(F^{(i)}) \in \Vo$ and can be uniquely written as 
% \[
% g(F^{(i)}) = \sum_{j=1}^{q^n} \beta_{i,j} \phi_j
% \]
% The equation (\ref{eq:ObsEqns}) can be re-written as the following linear system of equations
% \begin{align*}
%     \begin{bmatrix} \beta_{0,1} & \beta_{0,2}  & \dots & \beta_{0,q^n} \\ \vdots & \vdots &  \ddots & \vdots \\ \beta_{M,1} & \beta_{M,2} & \dots & \beta_{M,q^n} \\ \vdots & \vdots & \ddots & \vdots \\ \beta_{N-1,1} & \beta_{N-1,1} & \dots & \beta_{N-1,q^n}\end{bmatrix} \begin{bmatrix} \phi_1(x_0) \\ \phi_2(x_0) \\ \vdots \\ \phi_{q^n}(x_0)\end{bmatrix} = \begin{bmatrix} z(0) \\ z(1) \\ \vdots \\ z(N-1) \end{bmatrix}
% \end{align*}

% If the system is observable in the interval $0,\dots,M$, then it can be seen that the system of equations 
% \[
% g(F^{(i)})(x_0) = z(i) \quad \quad i = 0,\dots,M
% \]
% has an unique solution $x_0$ for all output sequences. This means the linear system of equations 
% \begin{align*}
%     \begin{bmatrix} \beta_{0,1} & \beta_{0,2}  & \dots & \beta_{0,q^n} \\ \vdots & \vdots &  \ddots & \vdots \\ \beta_{M,1} & \beta_{M,2} & \dots & \beta_{M,q^n} \end{bmatrix} \begin{bmatrix} \phi_1(x_0) \\ \phi_2(x_0) \\ \vdots \\ \phi_{q^n}(x_0)\end{bmatrix} = \begin{bmatrix} z(0) \\ z(1) \\ \vdots \\ z(M) \end{bmatrix}
% \end{align*}
% has a unique solution $x_0$. And the solution $x_0$ also satisfies (\ref{eq:}
\end{proof}
\textcolor{blue}{As a consequence of the above theorem, we have the following result about observability of a specific output sequence even when the system is unobservable.
\begin{corollary}
Any initial condition $x_0$ is observable iff it can be uniquely computed from the output sequence $Z_{N-1}$.
\end{corollary}}

\section{Conclusion}
In this paper, we developed an alternative linear approach to observability of nonlinear DSFF through the use of Koopman operator. Through this framework, we defined the LOR, linear output realization for a nonlinear system which can be viewed as the smallest dimensional linear system which can reproduce all the outputs of the original nonlinear system. The dimension of this linear system is defined through the construction of an invariant subspace of the Koopman operator. It is further established that the maximum number of outputs required to uniquely determine the initial condition from the corresponding output sequence is exactly equal to the dimension of the invariant subspace. Further directions
%This section discussed about theoretical formulations of observability of DSFF and we have a necessary and sufficient condition for the same using Theorem \ref{thm:obs_phat}. Given a dynamical system (\ref{eq:DSFF}), and its LOR (\ref{eq:LOR}), ascertaining the injectiveness of the map $\phat$ (\ref{eq:phat}) is a computationally hard problem given the basis functions $\psi_i(x)$. In the next section, we discuss an algorithm when the field $\ff$ is $\ff_2$ or the Boolean field.
